Large Language Model for Verilog Generation with Code-Structure-Guided Reinforcement Learning

Recent advancements in large language models (LLMs) have sparked significant interest in the automatic generation of Register Transfer Level (RTL) designs, particularly using Verilog. Current research on this topic primarily focuses on pre-training and instruction tuning, but the effectiveness of these methods is constrained by the limited availability of training data, as public Verilog code is far less abundant than software code. In particular, these methods struggle to effectively capture Verilog parallel code structures, which fundamentally differ from the imperative, sequential control flow typical in most software programming languages. This paper introduces VeriSeek, an LLM enhanced by reinforcement learning using a limited amount of high-quality training data to achieve high Verilog code generation performance. Our reinforcement learning approach employs code structure information as feedback signals to refine the pre-trained model, enabling it to effectively learn important patterns from Verilog code with parallel structures. Experiments show that VeriSeek outperforms state-of-the-art methods across multiple benchmarks.

==> tables/verilogeval_human.tex <==
\begin{table}[h]
\centering
\begin{threeparttable}
\setlength{\tabcolsep}{0.8pt}  % Reduced from 1pt to 0.8pt
\renewcommand\arraystretch{1.0}  % Reduced from 1.1 to 1.0
\footnotesize  % Changed from \small to \footnotesize for more compactness
\begin{tabular}{c@{\hspace{0.5em}}c@{\hspace{0.5em}}cccccc}  % Added custom spacing between first columns
\toprule
& & \multicolumn{6}{c}{\textbf{VerilogEval}} \\
\cmidrule(lr){3-8}
& & \multicolumn{3}{c}{\textbf{Eval-M(\%)}} & \multicolumn{3}{c}{\textbf{Eval-H(\%)}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
\multirow{-3}{*}{\textbf{Type}} &
\multirow{-3}{*}{\textbf{Model}} &
\p1 &
\p5 &
\p10 &
\p1 &
\p5 &
\p10
\\ \midrule

\multirow{2}{*}{\textbf{Closed}} & GPT-3.5 & 53.3 & 84.6 & 89.7 & 31.7 & 51.7 & 37.9 \\
& GPT-4 & 73.4 & 89.2 & 100.0 & 32.1 & 54.1 & 65.0 \\ \midrule

\multirow{4}{*}{\textbf{Open}} & Thakur-16B & 77.5 & 89.0 & 86.2 & 13.3 & 21.0 & 24.1 \\
& ChipGPT-7B & 32.3 & 40.4 & 38.9 & 17.8 & 29.0 & 34.3 \\
& ChipGPT-13B & 57.4 & 68.2 & 65.5 & 25.4 & 39.6 & 45.7 \\
& RTLCoder-7B & 66.9 & 88.4 & \textbf{96.6} & 25.3 & 40.5 & 48.3 \\ \midrule

\textbf{Base} & DeepSeek-6.7B & 65.3 & 88.2 & 89.3 & 21.4 & 31.6 & 39.3 \\ \midrule

\multirow{3}{*}{\textbf{Ours}} & \ours{}$_{PT}$-6.7B & 73.3 & 93.5 & 86.2 & 27.6 & 44.0 & 51.7 \\
& \ours$_{PTwC}$-6.7B & 83.6 & 95.0 & 92.2 & 31.5 & 46.3 & 51.7 \\
& \ours$_{PTwC+RL}$-6.7B & \textbf{84.1} & \textbf{95.2} & 93.1 & \textbf{33.4} & \textbf{52.3} & \textbf{--} \\ \bottomrule
\end{tabular}
\begin{tablenotes}\scriptsize
\item[*] All models have ~7B params, except ChipGPT-13B, Thakur-16B, GPT-3.5, and GPT-4.
\item[+] Bold: best metric (excluding GPT-4). P@N: Pass@N, M: Machine, H: Human.
\end{tablenotes}
\caption{Performance comparison of large language models for Verilog code generation. Our model after pretraining and reinforcement learning outperforms all other open-source models with a considerable gap, especially on functional metrics.}
\label{tab:verilogeval_rslt}
\end{threeparttable}
\end{table}

==> tables/verilogeval_machine.tex <==
% \begin{table}[h]
% \centering
% \caption{Comparison of model performance on VerilogEval-Machine benchmark, showing functional correctness metrics (\pass$1$, \pass$5$, \pass$10$) for our models against open-source SOTA models, GPT-3.5 and GPT-4. All metrics are reported in \%.}

% \begin{threeparttable}
% \setlength{\tabcolsep}{1pt}
% \renewcommand\arraystretch{1.0}
% \footnotesize
% \begin{tabular}{c@{\hspace{0.5em}}c@{\hspace{0.5em}}ccc}
% \toprule
% & & \multicolumn{3}{c}{\textbf{VerilogEval-Machine}} \\
% \cmidrule(lr){3-5}
% \multirow{-2}{*}{\textbf{Type}} &
% \multirow{-2}{*}{\textbf{Model}} &
% \pass{$1$} &
% \pass{$5$} &
% \pass{$10$}
% \\ \midrule

% \multirow{2}{*}{\textbf{Closed}} & GPT-3.5 & 46.7 & 69.1 & 74.1 \\
% & GPT-4 & 60.0 & 70.6 & 73.5 \\ \midrule

% \multirow{4}{*}{\textbf{Open}} & Thakur-16B & 44.0 & 52.6 & 59.2 \\
% & ChipGPT-7B & 47.6 & 57.1 & 61.9 \\
% & ChipGPT-13B & 58.6 & 69.4 & 71.1 \\
% & RTLCoder-7B & 61.2 & 76.5 & 81.8 \\ \midrule

% \textbf{Base} & DeepSeek-6.7B & 54.1 & 63.8 & 67.5 \\ \midrule

% \multirow{3}{*}{\textbf{Ours}} & \ours{}$_{PT}$-6.7B & 53.3 & 63.5 & 67.8 \\
% & \ours$_{PTwC}$-6.7B & 58.4 & 68.5 & 72.7 \\
% & \ours$_{PTwC+RL}$-6.7B & \colorbox{gray!25}{61.6} & \colorbox{gray!25}{76.9} & \colorbox{gray!25}{82.3} \\ \bottomrule
% \end{tabular}
% \begin{tablenotes}\scriptsize
% \item[+] \colorbox{gray!25}{Gray} background represents the best metric (excluding GPT-4).
% \end{tablenotes}
% \label{tab:verilogeval_rslt}
% \end{threeparttable}
% \end{table}



\begin{table}[h!]
\centering
\caption{Comparison of model performance on RTLLM2.0 benchmark, showing syntax and functional correctness metrics (\pass $1$, \pass $5$, \hitfive) for our models against open-source SOTA models, GPT-3.5 and GPT-4. All metrics are reported in \%.}
\begin{threeparttable}
\setlength{\tabcolsep}{1pt} % Reduced from 1.5pt to 1pt
\renewcommand\arraystretch{1.1} % Reduced from 1.2 to 1.1
\small % Added to make everything slightly smaller
\begin{tabular}{cc cccccc} % Reduced spacing between RTLLM sections from 2em to 1em
\toprule
& & \multicolumn{6}{c}{\textbf{VerilogEval}} \\
\cmidrule(lr){3-8}
& & \multicolumn{3}{c}{\textbf{Syntax}} & \multicolumn{3}{c}{\textbf{Function}} \\
\cmidrule(lr){3-5} \cmidrule(lr){6-8}
\multirow{-3}{*}{\textbf{Type}} &
\multirow{-3}{*}{\textbf{Model}} &
\p ${1}$ &
\p ${5}$ &
\hitfive &
\p ${1}$ &
\p ${5}$ &
\hitfive
\\ \midrule

& GPT-3.5 & - & - & - & 46.7 & 69.1 & 72.8 \\
\multirow{-2}{*}{\textbf{Closed}} & GPT-4 & - & - & - & 60.0 & 70.6 & 72.8 \\ \midrule

& Thakur-16B & - & - & - & 44.0 & 52.6 & 58.3 \\
& ChipGPT-7B & - & - & - & 47.6 & 57.1 & 61.3 \\
& ChipGPT-13B & - & - & - & 58.6 & 69.4 & 70.8 \\
\multirow{-4}{*}{\textbf{Open}} & RTLCoder-7B & - & - & - & 61.2 & 76.5 & 80.4 \\ \midrule

\textbf{Base} & DeepSeekCoder-6.7B & - & - & - & 54.1 & 63.8 & 65.9 \\ \midrule

& \ours{}$_{PT}$-6.7B & - & - & - & 53.3 & 63.5 & 65.2 \\
& \ours$_{PTwC}$-6.7B & - & - & - & 58.4 & 68.5 & 71.9 \\
\multirow{-3}{*}{\textbf{Ours}} & \ours$_{PTwC+RL}$-6.7B & - & - & - & \colorbox{gray!25}{61.6} & \colorbox{gray!25}{76.9} & \colorbox{gray!25}{82.3} \\ \bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
\item[+] \colorbox{gray!25}{Gray} background represents the best metric (excluding GPT-4).
\item[*] \p{$k$} represents \pass{$k$}.
\end{tablenotes}
\label{tab:rtllm}
\end{threeparttable}
\end{table}

